Bilinear CNNs for Fine-grained Visual Recognition

We present a simple and effective architecture for fine-grained visual recognition called Bilinear Convolutional Neural Networks (B-CNNs). These networks represent an image as a pooled outer product of features derived from two CNNs and capture localized feature interactions in a translationally invariant manner. B-CNNs belong to the class of orderless texture representations but unlike prior work they can be trained in an end-to-end manner. Our most accurate model obtains 84.1%, 79.4%, 86.9% and 91.3% per-image accuracy on the Caltech-UCSD birds [67], NABirds [64], FGVC aircraft [42], and Stanford cars [33] dataset respectively and runs at 30 frames-per-second on a NVIDIA Titan X GPU. We then present a systematic analysis of these networks and show that (1) the bilinear features are highly redundant and can be reduced by an order of magnitude in size without significant loss in accuracy, (2) are also effective for other image classification tasks such as texture and scene recognition, and (3) can be trained from scratch on the ImageNet dataset offering consistent improvements over the baseline architecture. Finally, we present visualizations of these models on various datasets using top activations of neural units and gradient-based inversion techniques. The source code for the complete system is available at http://vis-www.cs.umass.edu/bcnn.

==> spatial.tex <==
\begin{table}
\small
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{10pt}
\begin{center}
\begin{tabular}{l|c|c|c}
\textbf{model} & \textbf{birds} & \textbf{cars} & \textbf{aircrafts} \\ 
\hline 
B-CNN PCA & 75.75 & 81.47 & 78.37 \\ 
B-CNN PCA 4x4 & 76.34 & 83.53 &  79.42\\ 
B-CNN PCA 3x3 & 76.79 & 83.29 & 79.69 \\ 
B-CNN PCA (x,y) & 76.23 & 83.15 & 79.51 \\ 
\end{tabular} 
\end{center}
\caption{
\textbf{Effect of appending spatial information.} Spatial information is appended to one of feature channels VGG-M network which is then projected down to 64 dimensions in the B-CNN model. The position each feature is encoded as one-hot encoding of the bin index with bin size $4 \times 4$ and $3 \times 3$, or directly using normalized $x,y$-coordinates. The table reports the accuracy of the models using logistic regression classifier trained with flipping at training time.}
\label{tab:spatial_results}
\end{table}

The orderless pooling in the bilinear CNN models ignores the position of the features in the image. However, when the object is roughly localized in the image and modeling the position of the features can be useful. Indeed, appending normalized $x,y$-coordinates to the end of SIFT descriptors in the Fisher vector model has been shown to improve face recognition accuracy~\cite{parkhi14a-compact}. In our experiments we explore a similar strategy. We augment spatial information to the local descriptors in two ways -- (i) normalized $x,y$-coordinates of receptive field centers and (ii) one-hot encoding the bin index of the receptive field centers coordinates.

In order to encode the joint statistics of appearance and position we perform PCA on the spatially augmented features. We experiment with B-CNN [M,M] PCA models which are projected to 64 dimensions. The results after fine-tuning are shown in Table~\ref{tab:spatial_results}. The inclusion of spatial information improves accuracy, notably on cars which tend to be better localized in the images. Both the encoding schemes perform equally well.

